DISTAL: The Distributed Tensor Algebra Compiler

We introduce DISTAL, a compiler for dense tensor algebra that targets modern distributed and heterogeneous systems. DISTAL lets users independently describe how tensors and computation map onto target machines through separate format and scheduling languages. The combination of choices for data and computation distribution creates a large design space that includes many algorithms from both the past (e.g., Cannon's algorithm) and the present (e.g., COSMA). DISTAL compiles a tensor algebra domain specific language to a distributed task-based runtime system and supports nodes with multi-core CPUs and multiple GPUs. Code generated by DISTAL is competitive with optimized codes for matrix multiply on 256 nodes of the Lassen supercomputer and outperforms existing systems by between 1.8x to 3.7x (with a 45.7x outlier) on higher order tensor operations.

==> latexmkrc <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -o %D %O %S";

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for sharelatex
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    $qpdf //= "/usr/local/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf; # check that qpdf exists
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});
    my $status = system($qpdf, split(' ', $qpdf_opts), "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
    if (-e $rtex_file) {
        do_knitr($rtex_file);
    }
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}


==> scheduling-primitives.tex <==
\begin{figure*}
    \begin{tabular}{|c|}
        \hline
        split/divide \\
        \hline
        parallelize/distribute \\
        \hline
        precompute \\
        \hline
        fuse \\
        \hline
        reorder \\
        \hline
        \textbf{rotate} \\
        \hline
    \end{tabular}
    \caption{Scheduling Primitives}
    \label{fig:scheduling-primitives}
\end{figure*}


==> supported-algorithms.tex <==
\begin{figure*}
    \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{Matrix-Multiply Algorithms} \\
        \hline
        Cannon's Algorithm~\cite{cannon} & 2-D Systolic \\
        \hline
        PUMMA~\cite{pumma} & 2-D Systolic and Broadcast \\
        \hline
        SUMMA~\cite{summa} & 2-D Broadcast \\
        \hline
        Johnson's Algorithm~\cite{johnson} & 3-D reduction \\
        \hline
        Solomonik's 2.5D Algorithm~\cite{solomonikMM} & 3-D reduction with inter-plane Cannon's \\
        \hline
        COSMA~\cite{cosma} & Intelligent selection of distribution grid to minimize communication \\
        \hline
        \hline
        \multicolumn{2}{|c|}{Higher Order Tensor Algorithms} \\
        \hline
        Ballard's MTTKRP~\cite{ballardmttkrp} & 3-D decomposition with in-place tensor \\
        \hline
    \end{tabular}
    \caption{Algorithms. TODO (rohany): I need to come up with better ways to talk give a summary of these.}
    \label{fig:algorithms}
\end{figure*}


